Knowledge Guided Named Entity Recognition for BioMedical Text

In this work, we formulate the NER task as a multi-answer knowledge guided QA task (KGQA) which helps to predict entities only by assigning B, I and O tags without associating entity types with the tags. We provide different knowledge contexts, such as, entity types, questions, definitions and examples along with the text and train on a combined dataset of 18 biomedical corpora. This formulation (a) enables systems to jointly learn NER specific features from varied NER datasets, (b) can use knowledge-text attention to identify words having higher similarity to provided knowledge, improving performance, (c) reduces system confusion by reducing the prediction classes to B, I, O only, and (d) makes detection of nested entities easier. We perform extensive experiments of this KGQA formulation on 18 biomedical NER datasets, and through experiments we note that knowledge helps in achieving better performance. Our problem formulation is able to achieve state-of-the-art results in 12 datasets.

==> temp.tex <==




% We show  the learning curves  for each of the different knowledge  types in Figure \ref{fig:mtlearning}. It can be seen that the  performance of the model increases rapidly and then slows down for each of the knowledge types. We can infer that the model can achieve quite a good performance(\char`\~84\%) with just 5\% of training data but needs much more data to achives the state-of-the-art performance. As the training  samples goes beyond 5\%, the precision, recall and the F1-scores for knowledge type \textit{Question} clearly separates itself from the remaining types. The best Precision, Recall and F1-Score on validation data are 89.68, 88.96, 89.32 for Question as knowledge type, 85.14, 85.94, 85.54 for definition, 87.97, 87.44, 87.70 for entity type and 88.44, 87.48, 87.95 for examples as knowledge context respectively. It can also be seen that the learning curve of BERT-CNN is similar to BioBERT. MimicBERT however fails to learn as well as the other two models which explain the reduced performance of MimicBERT as discussed earlier.




% % such as in Named Entity Recognition (CoNLL-2003 \cite{conll2003}, OntoNotes \cite{inbook1}, etc) and Relation Extraction (SEMEval-2010 \cite{hendrickx-etal-2010-semeval}, TACRED \cite{tacred}, etc


% % AnatEM, 2012-i2b2(Occurance, clinical-department event, evidential event), BIONLP11ID(Organism, Regular-Operon), Linnaeus(Species) and  JNLPBA(Cell-Type, DNA, RNA)


% Here, we show the importance of using  knowledge with our model and our task formulation by comparing  the performance  when with question as knowledge and with no knowledge at all. Since our NER task formulation does not require mentions of specific entity-types apart from the knowledge context, we execute this experiment for each of the six common named entity groups namely, \textit{gene/protein, chemical, disease, test, treatment, problem}. We choose these six entities since they appear in more than one dataset. We keep the other parameters of BERT-CNN model same.
% % For gene/protein we use 10 datasets (BC2GM, BIONLP09, BIONLP11EPI, BIONLP11ID, BIONLP13CG, BIONLP13PC, BIONLP13GE, CRAFT, ExPTM, JNLPBA) and for chemical we use 6 datasets BC4CHEMD, BC5CDR, BIONLP11ID, BIONLP13CG, BIONLP13PC. However there are only 2 datasets(NCBIDisease, BC5CDR) where diseases can be found. Finally for the each of problem, treatment and test we use all three i2b2 datasets (2010, 2011, 2012).
% From the Table \ref{tab:kvsnok}, we show that the use of each knowledge types gives a boost in performance across  all the six  entity types than when no knowledge is used. This shows the importance of knowledge. It can be seen that the entity type ``gene/protein'' which is present in 10 datasets suffers most when no knowledge is provided by almost 15\%. For ``chemical" the  drop is by 3\% and for disease it is around 1\% which is because it is present in only two datasets and has small number of samples.  We believe that knowledge(especially Question) helps guide the model to resolve the variations of vast domain of gene/protein.




% \subsection{Error Analysis \textcolor{red}{TODO}}



% We analyze for a few samples, how the attention heads help the BioBERT+CNN model with question as knowledge to choose the answer using the BERT visualization  tool \cite{vig2019transformervis}. In Figure \ref{fig:viz}, for  a  text, ``\textit{Percocet and morphine sulfate for pain.}" and knowledge context ``\textit{What is the problem mentioned in the text ?}", it can be seen that each of the words of the question attends to the correct answer option ``\textit{pain}" with high confidence although there are other entities present in the text. We also observe for CRAFT, the knowledge in the form of Examples help, but definitions under perform. This indicates better knowledge formulation can improve performance even further.
% In Table \ref{tab:sota} we compare our models with baseline models of BioBERT and MimicBERT trained using our task formulation, and the current state-of-the-art models. It shows our task formulation considerably improves the state-of-the-art for these tasks. We identify four reasons for improvements in accuracy. First, making the task to have no overlapping entities. Second, reducing the number of classes for prediction. Third, the sheer size of the dataset which enables the system to learn more NER specific features. Last, a CNN model over the BERT language model which enables to combine contextual features to perform better NER predictions. 



% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \begin{table*}[!htb]
% % \centering
% % \scriptsize
% % \resizebox{\textwidth} {!}{
% % \begin{tabular}{l|cccc|cccc|cccc}
% % \toprule
% % \multirow{2}{*}{\textbf{DATASET}} & \multicolumn{3}{c|}{\textbf{ENTITY-TYPE}} & \multicolumn{3}{c|}{\textbf{QUESTION}} & \multicolumn{3}{c|}{\textbf{DEFINITION}} & \multicolumn{3}{c}{\textbf{EXAMPLE}} \\ \cline{2-13} 
% %                          & \textbf{P}       & \textbf{R}       & \textbf{F}       & \textbf{P}        & \textbf{R}        & \textbf{F}       & \textbf{P}         & \textbf{R}        & \textbf{F}        & \textbf{P}        & \textbf{R}       & \textbf{F}       \\ \hline

% % \shortstack{\textbf{\texttt{ANATEM}}} &88.60&87.30&87.94&88.79&88.02&\textbf{88.40}&88.39&86.50&87.44&88.88&87.80&88.33  \\ 
% % \shortstack{\textbf{\texttt{BC2GM}}}  &81.66&81.98&81.82&82.35&82.75&\textbf{82.54}&80.76&80.60&80.68&81.65&80.93&81.29\\ 
% % \shortstack{\textbf{\texttt{BC4CHEMD }}} &90.02&88.56&89.29&91.52&90.23&\textbf{90.87}&89.64&87.28&88.45&90.34&87.97&89.14  \\ 
% % \shortstack{\textbf{\texttt{BC5CDR}}} &87.96&86.51&87.23&89.26&88.34&\textbf{88.80}&87.51&85.85&86.67&87.70&86.15&86.92     \\ 
% % \shortstack{\textbf{\texttt{BIONLP09}}} &88.81&89.08&88.95&90.41&91.86&\textbf{91.12}&50.47&69.71&58.54&89.79&88.84&89.31   \\ 
% % \shortstack{\textbf{\texttt{BIONLP11EPI}}} &86.98&83.05&84.96&87.91&85.93&\textbf{86.90}&78.13&82.56&80.28&87.09&82.50&84.73 \\ 
% % \shortstack{\textbf{\texttt{BIONLP11ID}}} &83.91&81.77&82.81&85.38&83.33&\textbf{84.17}&82.00&81.38&81.66&84.02&81.57&82.77   \\ 
% % \shortstack{\textbf{\texttt{BIONLP13CG}}} &85.74&83.60&84.61&89.08&86.54&\textbf{87.78}&84.37&82.87&83.53&87.48&86.07&86.75 \\ 
% % \shortstack{\textbf{\texttt{BIONLP13GE}}}  &79.78&83.96&81.81&82.74&87.20&\textbf{84.91}&69.58&79.23&74.07&79.62&83.27&81.40   \\ 
% % \shortstack{\textbf{\texttt{BIONLP13PC}}} &88.87&89.34&89.10&89.52&91.11&\textbf{90.30}&87.42&88.16&87.78&89.13&89.48&89.30   \\ 
% % \shortstack{\textbf{\texttt{CRAFT}}}  &86.00&84.68&85.33&87.85&87.15&\textbf{87.50}&82.02&83.88&82.93&88.52&88.06&88.28\\ 
% % \shortstack{\textbf{\texttt{EX-PTM}}} &83.46&82.60&83.03&83.90&84.95&\textbf{84.42}&74.43&82.18&78.11&83.42&82.10&82.75 \\ 
% % \shortstack{\textbf{\texttt{JNLPBA}}} &70.76&77.40&73.93&76.20&80.90&\textbf{78.48}&66.63&71.52&68.96&70.72&78.42&74.36 \\ 
% % \shortstack{\textbf{\texttt{LINNAEUS}}} & 89.67&86.34&87.96&88.94&87.21&\textbf{88.16}&87.81&85.06&86.40&90.26&88.46&89.34 \\ 
% % \shortstack{\textbf{\texttt{NCBI-DISEASE}}}  &86.35&90.01&88.14&87.17&90.12&\textbf{88.62}&86.69&88.91&87.78&86.32&89.10&87.68 \\ 
% % \shortstack{\textbf{\texttt{2010-i2b2}}}  &93.30&93.99&93.64&94.85&95.62&\textbf{95.24}&92.73&93.75&93.24&93.18&94.23&93.70 \\ 
% % \shortstack{\textbf{\texttt{2011-i2b2}}}   &92.97&92.03&92.49&93.81&94.05&\textbf{93.93}&92.50&91.85&92.17&93.81&93.24&93.52  \\ 
% % \shortstack{\textbf{\texttt{2012-i2b2}}}    &80.16&81.62&80.85&83.64&84.89&\textbf{84.25}&78.24&81.43&79.75&63.15&81.09&70.66 \\ \hline
% % \end{tabular}
% % }
% % \caption{Precision(P), Recall(R) and F-Measure(F) for selected datasets using the best performing BERT-CNN model using different knowledge types, which are, Entity Type, Question, Definition  and Examples.  Best Exact Match F1 scores are in Bold. The values in the table are mean of three seeds 42, 512, 1024. The full table can be found in the Supplemental Materials with the standard deviations}
% % \label{tab:my-table}
% % \end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \begin{table*}[!htb]
% % \small
% % \begin{tabular}{|l|l|l|l|l|l|l|l|}
% % \hline
% % \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}MODELS\\ DATASETS\end{tabular}} & \multicolumn{4}{c|}{BASELINE}                                                                                        & \multicolumn{3}{c|}{OUR}                                                                      \\ \cline{2-8} 
% %                                                                           & \multicolumn{1}{c|}{BioBERT} & \multicolumn{1}{c|}{MimicBERT} & \multicolumn{1}{c|}{MRC} & \multicolumn{1}{c|}{SOTA} & \multicolumn{1}{c|}{BioBERT} & \multicolumn{1}{c|}{MimicBERT} & \multicolumn{1}{c|}{BERT-CNN} \\ \hline
% % ANATEM                                                                     &                              &                                &                          &                           &                              &                                &                               \\ \hline
% % BC2GM                                                                      &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% %                                                                           &                              &                                &                          &                           &                              &                                &                               \\ \hline
% % \end{tabular}
% % \caption{
% % Precision(P), Recall(R) and F-Measure(F) for selected datasets using multiple models. SOTA scores are from \cite{si2019enhancing,lee2019biobert,beltagy2019scibert}. Few current SOTA scores are for BERT Large, ours though use BERT Base. i2b2 scores are compared with \cite{si2019enhancing}. \textcolor{red}{TODO}
% %     }
% % \label{tab:sota}
% % \end{table*}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}



% % \begin{table}
% %         \centering
% %         \scriptsize
% %         \resizebox{\columnwidth} {!}{
% %         % \resizebox{1.0\columnwidth}{!}{
% %         \begin{tabular}{c |c |c c c }
% %             \toprule 
            
% %             \multirow{1}{*}{\textbf{DATASET}}&
% %             \multirow{1}{*}{\textbf{MODEL}}
% %             % & \multicolumn{3}{c}{\textbf{Context$_1$}}\\ \cline{3-5}
% %             &  \multicolumn{1}{c}{\textbf{P}}
% %             & \multicolumn{1}{c}{\textbf{R}}
% %             & \multicolumn{1}{c}{\textbf{F}}\\
% %              \hline
             
% %              \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{ANATEM}}}}}
% %             & B\textsc{ioBERT} &89.68  & 88.57 &89.12 \\ 
% %             & M\textsc{imicBERT} &86.86&	85.73& 86.29 \\ 
% %             & S\textsc{OTA} & - & - & \textbf{91.61} \\ 
% %             % & B\textsc{ERTCNN} &92.07 & 91.01 & \textbf{91.54}\\ 
% %             & B\textsc{ERTCNN} &88.79&88.02&88.40\\
% %              \hline
             
% %              \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BC2GM}}}}}
% %             & B\textsc{ioBERT} &82.47 & 83.36 & \textbf{82.91}  \\ 
% %             & M\textsc{imicBERT} &81.22&	81.40&	81.31 \\ 
% %             & S\textsc{OTA} & - & - & 81.69 \\ 
% %             & B\textsc{ERTCNN} & 82.35&82.75&82.54\\ 
% %              \hline
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BC4CHEMD}}}}}
% %             & B\textsc{ioBERT} &91.93 & 91.11 & \textbf{91.52}  \\ 
% %             & M\textsc{imicBERT} &89.47&	88.86&	89.16 \\ 
% %             & S\textsc{OTA} & - & - & 89.37 \\ 
% %             & B\textsc{ERTCNN} &91.52&90.23&90.87\\ 
% %              \hline
             
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BC5CDR}}}}}
% %             & B\textsc{ioBERT} &89.63 & 88.80 &\textbf{ 89.21}  \\ 
% %             & M\textsc{imicBERT} &88.25&	86.78	&87.51 \\ 
% %             & S\textsc{OTA} & - & - & 86.23 \\ 
% %             & B\textsc{ERTCNN} & 89.26&88.34&88.8\\ 
% %              \hline
             
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BIONLP09}}}}}
% %             & B\textsc{ioBERT} &91.35 & 92.21 & \textbf{91.78} \\ 
% %             & M\textsc{imicBERT} &89.19&	91.41	&90.29 \\ 
% %             & S\textsc{OTA} & - & - & 84.20 \\ 
% %             & B\textsc{ERTCNN} &90.41&91.86&91.12\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BIONLP11EPI}}}}}
% %             & B\textsc{ioBERT} &88.26 & 86.77 & \textbf{87.51}  \\ 
% %             & M\textsc{imicBERT} &88.015&	82.19	&85.00 \\ 
% %             & S\textsc{OTA} & - & - & 78.86 \\ 
% %             & B\textsc{ERTCNN} &87.91&85.93&86.9\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BIONLP11ID}}}}}
% %             & B\textsc{ioBERT} &86.34&85.58&\textbf{85.96 } \\ 
% %             & M\textsc{imicBERT} &83.12&	81.78	&82.45 \\ 
% %             & S\textsc{OTA} & - & - & 82.26 \\ 
% %             & B\textsc{ERTCNN} &85.38&83.33&84.17\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BIONLP13CG}}}}}
% %             & B\textsc{ioBERT} &87.18 & 87.28 & 87.23  \\ 
% %             & M\textsc{imicBERT} &85.08&	85.37	&85.23 \\ 
% %             & S\textsc{OTA} & - & - & 78.90 \\ 
% %             & B\textsc{ERTCNN} &89.08&86.54&\textbf{87.78}\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BIONLP13GE}}}}}
% %             & B\textsc{ioBERT} &82.28&86.58&84.38  \\ 
% %             & M\textsc{imicBERT} &81.61&86.28&83.88 \\ 
% %             & S\textsc{OTA} & - & - & 78.58 \\ 
% %             & B\textsc{ERTCNN} & 82.74&87.2&\textbf{84.91}\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{BIONLP13PC}}}}}
% %             & B\textsc{ioBERT} &90.14&92.09&\textbf{91.11} \\ 
% %             & M\textsc{imicBERT} &87.62&89.63&88.61 \\ 
% %             & S\textsc{OTA} & - & - & 81.92 \\ 
% %             & B\textsc{ERTCNN} &89.52&91.11&90.30\\ 
% %              \hline
             
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{CRAFT}}}}}
% %             & B\textsc{ioBERT} &86.99 & 87.11 & 87.05  \\ 
% %             & M\textsc{imicBERT} & 86.12	&84.74	&85.43 \\ 
% %             & S\textsc{OTA} & - & - & 79.55 \\ 
% %             & B\textsc{ERTCNN}& 87.85&87.15&\textbf{87.50}\\ 
% %              \hline
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{ExPTM}}}}}
% %             & B\textsc{ioBERT} &85.97 & 85.30 & \textbf{85.64 }\\ 
% %             & M\textsc{imicBERT} & 84.09	&81.34	&82.69 \\ 
% %             & S\textsc{OTA} & - & - & 74.90\\ 
% %             & B\textsc{ERTCNN} &83.9&84.95&84.42\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{JNLPBA}}}}}
% %             & B\textsc{ioBERT} &76.12&82.15&\textbf{79.02} \\ 
% %             & M\textsc{imicBERT} &74.97&80.79&77.77 \\ 
% %             & S\textsc{OTA} & - & - & 78.58 \\ 
% %             & B\textsc{ERTCNN} &76.20&80.90&78.48\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{LINNAEUS}}}}}
% %             & B\textsc{ioBERT} &88.34&88.40&88.37  \\ 
% %             & M\textsc{imicBERT} &86.31&85.10&85.70 \\ 
% %             & S\textsc{OTA} & - & - & \textbf{95.68 }\\ 
% %             & B\textsc{ERTCNN} &88.94&87.21&88.16\\ 
% %              \hline
             
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{NCBI-Disease}}}}}
% %             & B\textsc{ioBERT} &87.55 & 90.67 & \textbf{89.05}  \\ 
% %             & M\textsc{imicBERT} &86.82&	88.80	&87.80\\ 
% %             & S\textsc{OTA} & - & - & 88.60 \\ 
% %             & B\textsc{ERTCNN} &87.17&90.12&88.62\\ 
% %              \hline
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{2010-I2B2}}}}}
% %             & B\textsc{ioBERT} &89.16 & 92.47 & 90.79 \\ 
% %             & M\textsc{imicBERT} &94.85&	95.76	&\textbf{95.30} \\ 
% %             & S\textsc{OTA} & - & - & 90.25 \\ 
% %             & B\textsc{ERTCNN} &94.85&95.62&95.24\\ 
% %              \hline
              
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{2011-I2B2}}}}}
% %             & B\textsc{ioBERT} &93.88&94.15&94.02  \\ 
% %             & M\textsc{imicBERT} &94.18&94.30&\textbf{94.24} \\ 
% %             & S\textsc{OTA} & - & - & - \\ 
% %             & B\textsc{ERTCNN} & 93.81&94.05&93.93\\ 
% %              \hline
             
             
% %             \multirow{3}{*}{
% %                 \rotatebox[origin=c]{0}{
% %                     \shortstack{\textbf{\texttt{2012-I2B2}}}}}
% %             & B\textsc{ioBERT} &74.00 & 70.90 & 72.42 \\ 
% %             & M\textsc{imicBERT} &81.57&	84.76	& 83.13 \\ 
% %             & S\textsc{OTA} & - & - & 80.91 \\ 
% %             & B\textsc{ERTCNN}&83.64&84.89&\textbf{84.25}\\ 
% %              \hline
             
% %             \end{tabular}
% %             }
% %             \caption{
% %             Precision(P), Recall(R) and F-Measure(F) for selected datasets using multiple models. SOTA scores are from \cite{si2019enhancing,lee2019biobert,beltagy2019scibert}. Few current SOTA scores are for BERT Large, ours though use BERT Base. i2b2 scores are compared with \cite{si2019enhancing}.
% %                 }
% %             \label{tab:sota}
% %         \end{table}  
        
        
        
% % \begin{table*}[t]
% % \centering
% % \tiny
% % \resizebox{\textwidth} {!}{
% % \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% % \toprule
% % \multicolumn{2}{|c|}{MODELS$\downarrow$  / DATASETS$\xrightarrow{}$} & ANATEM     & BC2GM & BC4CHEMD & BC5CDR & BIONLP09 & BIONLP11EPI  & BIONLP11ID & BIONLP13CG & BIONLP13GE \\ \hline
% % \multirow{3}{*}{BASELINE}  & BioBERT    &   89.63\;	89.32\;	89.47         &       &          &        &          &              &            &            &            \\ \cline{2-11} 
% %                           & MimicBERT  &            &       &          &        &          &              &            &            &            \\ \cline{2-11} 
% %                           & BERT-MRC   &            &       &          &        &          &              &            &            &            \\ \hline
% % \multicolumn{2}{|c|}{SOTA}              &            &       &          &        &          &              &            &            &            \\ \hline
% % OURS                       & BioBERT    &            &       &          &        &          &              &            &            &            \\ \hline
% %                           & MimicBERT  &            &       &          &        &          &              &            &            &            \\ \hline
% %                           & BERT-CNN   &            &       &          &        &          &              &            &            &            \\ 
% % \toprule
% % \multicolumn{2}{|c|}{MODELS $\downarrow$ / DATASETS $\xrightarrow{}$} & BIONLP13PC & CRAFT & EX-PTM   & JNLPBA & LINNAEUS & NCBI-DISEASE & 2010 i2b2  & 2011 i2b2  & 2012 i2b2  \\ \hline
% % \multirow{3}{*}{BASELINE}  & BioBERT    &   11 \;  22 \;33     &       &          &        &          &              &            &            &            \\ \cline{2-11} 
% %                           & MimicBERT  &            &       &          &        &          &              &            &            &            \\ \cline{2-11} 
% %                           & BERT-MRC   &            &       &          &        &          &              &            &            &            \\ \hline
% % \multicolumn{2}{|c|}{SOTA}              &            &       &          &        &          &              &            &            &            \\ \hline
% % \multirow{3}{*}{OURS}      & BioBERT    &            &       &          &        &          &              &            &            &            \\ \cline{2-11} 
% %                           & MimicBERT  &            &       &          &        &          &              &            &            &            \\ \cline{2-11} 
% %                           & BERT-CNN   &            &       &          &        &          &              &            &            &            \\ \hline
% % \end{tabular}
% % }
% % \caption{
% % Precision(P), Recall(R) and F-Measure(F) for selected datasets using multiple models. The Baseline and SOTA scores are from \cite{si2019enhancing,lee2019biobert,beltagy2019scibert,crichton2017neural}. Few current SOTA scores are for BERT Large, ours though use BERT Base. i2b2 scores are compared with \cite{si2019enhancing}. \textcolor{red}{TODO}
% %     }
% % \label{tab:sota}
% % \end{table*}


% \begin{table*}[t]
%         \centering
%         \scriptsize
%         \resizebox{1.7\columnwidth} {!}{
%         % \resizebox{1.0\columnwidth}{!}{
%         \begin{tabular}{c c c c c  c c c  c c c c c c}
%             \toprule 
%             %  & & \multicolumn{3}{c}{\underline{\textbf{Concept$_1$}}} & \multicolumn{3}{c}{\underline{\textbf{Concept$_2$}}} & \multicolumn{3}{c}{\underline{\textbf{Concept$_3$}}}\\
            
%             % %% E2C
%             % \textbf{Dataset} & \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} &\multicolumn{1}{c}{\textbf{F}}& \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} &\multicolumn{1}{c}{\textbf{F}}& \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} &\multicolumn{1}{c}{\textbf{F}}\\
%             % \hline
            
%             \multirow{2}{*}{\textbf{\texttt{Dataset}}}&
%             \multirow{2}{*}{\textbf{\texttt{Models}}}
%             & \multicolumn{3}{c}{\textbf{Entity Type}} & \multicolumn{3}{c}{\textbf{Question}} & \multicolumn{3}{c}{\textbf{Definition}}& \multicolumn{3}{c}{\textbf{Example}}\\ \cline{3-14}
%             & & \multicolumn{1}{c}{\textbf{P}}
%             & \multicolumn{1}{c}{\textbf{R}}
%             & \multicolumn{1}{c}{\textbf{F}}
%             & \multicolumn{1}{c}{\textbf{P}}
%             & \multicolumn{1}{c}{\textbf{R}}
%             & \multicolumn{1}{c}{\textbf{F}}
%             & \multicolumn{1}{c}{\textbf{P}}
%             & \multicolumn{1}{c}{\textbf{R}}
%             & \multicolumn{1}{c}{\textbf{F}}
%             & \multicolumn{1}{c}{\textbf{P}}
%             & \multicolumn{1}{c}{\textbf{R}}
%             & \multicolumn{1}{c}{\textbf{F}}\\
%              \hline
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{AnatEM}}}}}
%             & B\textsc{ioBERT} &89.49 & 87.02 & 88.24 & 89.68 & 88.57 & 89.12 & 88.42 & 88.02 & 88.22 & 90.29 & 89.43 & 89.85\\ 
%             & M\textsc{imicBERT} & 86.25 & 84.53 & 85.38 & 86.86 & 85.73 & 86.29 & 85.82 & 82.13 & 83.93 & 87.05 & 86.5 & 86.8\\ 
%             & S\textsc{OTA} & - & - & \textbf{91.61}& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 89.43 & 87.54 & 88.47 & 88.81 & 89.12 & 88.96 & 89.03 & 87.23 & 88.13 & 89.41 & 88.69 & 89.05\\ 
%              \hline
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BC2GM}}}}}
%             & B\textsc{ioBERT} & 81.63 & 82.37 & 81.99 & 82.47 & 83.36 & 82.91 & 81.3 & 81.75 & 81.52 & 81.82 & 82.28 & 82.05 \\ 
%             & M\textsc{imicBERT} & 79.56 & 79.57 & 79.56 & 81.22 & 81.4 & 81.31 & 78.53 & 77.88 & 78.21 & 78.44 & 79.55 & 78.99\\ 
%             & S\textsc{OTA} & - & - & 81.69& - & -& - & -&- & -& - & -&-\\ 
%             & B\textsc{ERTCNN} & 81.79 & 82.06 & 81.93 & 82.89 & 83.39 & \textbf{83.14} & 80.62 & 80.21 & 80.42 & 82.37 & 82.29 & 82.33\\ 
%              \hline
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BC4CHEMD}}}}}
%             & B\textsc{ioBERT} & 90.14 & 89.53 & 89.83 & 91.93 & 91.11 & 91.52 & 89.64 & 88.23 & 88.93 & 90.15 & 89.27 & 89.71\\ 
%             & M\textsc{imicBERT} & 87.88 & 85.79 & 86.83 & 89.47 & 88.86 & 89.16 & 86.32 & 84.21 & 85.25 & 86.71 & 86.01 & 86.36\\ 
%             & S\textsc{OTA} & - & - & 89.37 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 89.83 & 88.89 & 89.36 & 92.07 & 91.01 & \textbf{91.54 }& 89.77 & 87.15 & 88.44 & 90.57 & 89.27 & 89.92\\ 
%              \hline
             
            
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BC5CDR}}}}}
%             & B\textsc{ioBERT} & 87.55 & 87.27 & 87.41 & 89.63 & 88.8 & 89.21 & 87.66 & 86.3 & 86.97 & 88.4 & 87.48 & 87.94\\ 
%             & M\textsc{imicBERT} & 86.29 & 84.85 & 85.56 & 88.25 & 86.78 & 87.51 & 85.54 & 83.97 & 84.75 & 86.31 & 84.35 & 85.31\\ 
%             & S\textsc{OTA} & - & - & 86.23& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 88.25 & 86.13 & 87.18 & 90.09 & 89.16 & \textbf{89.62} & 88.07 & 86.12 & 87.08 & 88.49 & 86.62 & 87.55\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{ BioNLP09}}}}}
%             & B\textsc{ioBERT} & 88.56 & 88.88 & 88.72 & 91.35 & 92.21 & \textbf{91.78} & 50.03 & 69.19 & 58.07 & 89.81 & 88.92 & 89.36\\ 
%             & M\textsc{imicBERT} & 88.26 & 88.46 & 88.36 & 89.19 & 91.41 & 90.29 & 49.13 & 70.51 & 57.91 & 88.02 & 89.66 & 88.83\\ 
%             & S\textsc{OTA} & - & - & 84.20 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 88.91 & 88.99 & 88.95 & 90.16 & 91.52 & 90.83 & 49.26 & 70.73 & 58.07 & 89.75 & 88.97 & 89.36\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BioNLP11EPI}}}}}
%             & B\textsc{ioBERT} & 86.95 & 82.78 & 84.822 & 88.26 & 86.77 & 87.51 & 78.49 & 83.85 & 81.08 & 87.55 & 84.91 & 86.21\\ 
%             & M\textsc{imicBERT} & 84.65 & 79.59 & 82.04 & 88.01 & 82.19 & 85 & 73.16 & 79.87 & 76.37 & 83.84 & 79.59 & 81.66\\ 
%             & S\textsc{OTA} & - & - & 78.86& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 87 & 83.15 & 85.03 & 88.58 & 87.4 & \textbf{87.99} & 77.56 & 83.53 & 80.44 & 87.55 & 83.32 & 85.38\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{ BioNLP11ID}}}}}
%             & B\textsc{ioBERT} & 81.1 & 81.14 & 81.12 & 86.34 & 85.58 & 85.96 & 83.03 & 81.82 & 82.42 & 82.42 & 83.74 & 83.08\\ 
%             & M\textsc{imicBERT} & 79.98 & 78.19 & 79.078 & 83.12 & 81.78 & 82.45 & 77.63 & 77.85 & 77.74 & 77.38 & 78.35 & 77.87\\ 
%             & S\textsc{OTA} &  - & - & 82.26 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 81.91 & 83.01 & 82.45 & 86.6 & 85.35 & \textbf{85.97} & 79.43 & 83.17 & 81.26 & 82.85 & 82.2 & 82.52\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BioNLP13CG}}}}}
%             & B\textsc{ioBERT} & 82.99 & 84.31 & 83.65 & 87.18 & 87.28 & 87.23 & 80.73 & 84.25 & 82.45 & 85.38 & 87.91 & 86.62\\ 
%             & M\textsc{imicBERT} & 77.28 & 82.4 & 79.76 & 85.08 & 85.37 & 85.23 & 75.95 & 80.17 & 78 & 80.54 & 84.96 & 82.69\\ 
%             & S\textsc{OTA} &  - & - & 78.90 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 81.24 & 84.79 & 82.98 & 87.97 & 87.26 & \textbf{87.62} & 78.47 & 84.21 & 81.24 & 84.57 & 87.11 & 85.82\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BioNLP13GE}}}}}
%             & B\textsc{ioBERT} &78.27 & 83.98 & 81.03 & 82.28 & 86.58 & \textbf{84.38} & 71.25 & 81.65 & 76.1 & 78.77 & 83.55 & 81.09\\ 
%             & M\textsc{imicBERT} & 77.41 & 82.95 & 80.08 & 81.61 & 86.28 & 83.88 & 66.66 & 77.72 & 71.77 & 77.04 & 84.42 & 80.56\\ 
%             & S\textsc{OTA} &  - & - & 78.58& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 80.86 & 84.72 & 82.747 & 81.82 & 86.26 & 83.98 & 68.64 & 81.32 & 74.44 & 80.26 & 84.48 & 82.32\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{BioNLP13PC}}}}}
%             & B\textsc{ioBERT} & 87.02 & 90.10 & 88.53 & 90.14 & 92.09 & \textbf{91.11} & 87.29 & 88.87 & 88.07 & 89.33 & 91.11 & 90.21\\ 
%             & M\textsc{imicBERT} & 85.96 & 88.13 & 87.03 & 87.62 & 89.63 & 88.61 & 84.95 & 85.87 & 85.4 & 86.84 & 87.66 & 87.25\\ 
%             & S\textsc{OTA} &  - & - & 81.92 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 88.14 & 89.77 & 88.95 & 89.03 & 91.87 & 90.43 & 86.23 & 88.94 & 87.56 & 88.95 & 90.58 & 89.76\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{CRAFT}}}}}
%             & B\textsc{ioBERT} & 85.2 & 85.59 & 85.4 & 86.99 & 87.11 & 87.05 & 82.84 & 84.1 & 83.47 & 88.18 & 88.61 & 88.39\\ 
%             & M\textsc{imicBERT} & 82.77 & 82.42 & 82.6 & 86.12 & 84.74 & 85.43 & 78.27 & 80.12 & 79.19 & 85.01 & 87.14 & 86.06\\ 
%             & S\textsc{OTA} &  - & - & 79.55 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 85.26 & 85.57 & 85.41 & 88.07 & 88.19 & 88.13 & 80.72 & 84.19 & 82.42 & 88.00 & 89.18 & \textbf{88.58}\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{EXPTM}}}}}
%             & B\textsc{ioBERT} & 82.74 & 84.31 & 83.52 & 85.97 & 85.3 &\textbf{ 85.64 }& 74.52 & 83.57 & 78.79 & 84.02 & 84.44 & 84.23\\ 
%             & M\textsc{imicBERT} & 82.007 & 78.15 & 80.03 & 84.09 & 81.34 & 82.69 & 68.92 & 77.32 & 72.88 & 81.04 & 79.75 & 80.39\\ 
%             & S\textsc{OTA} &  - & - & 74.90 & - & -& - & -&- & -& - & -&-\\
%             & C\textsc{NNBERT} &84.64 & 82.67 & 83.65 & 83.718 & 85.738 & 84.71 & 74.012 & 83.96 & 78.67 & 83.43 & 82.6 & 83.01\\ 
%              \hline
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{JNLPBA}}}}}
%             & B\textsc{ioBERT} & 70.12 & 77.88 & 73.8 & 76.127 & 82.15 & \textbf{79.02} & 66.11 & 70.33 & 68.16 & 69.14 & 79.54 & 73.98\\ 
%             & M\textsc{imicBERT} & 68.63 & 76.78 & 72.48 & 74.97 & 80.79 & 77.77 & 65.42 & 71.41 & 68.28 & 67.17 & 78.06 & 72.21\\ 
%             & S\textsc{OTA} &-  &- &78.58 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 69.78 & 77.77 & 73.55 & 76.04 & 81.632 & 78.73 & 64.45 & 73.38 & 68.63 & 69.29 & 79.25 & 73.94\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{Linnaeus}}}}}
%             & B\textsc{ioBERT} & 87 & 87.49 & 87.24 & 88.34 & 88.4 & 88.37 & 86.8 & 86.94 & 86.88 & 90.32 & 89.88 & 90.10\\ 
%             & M\textsc{imicBERT} &80.27 & 83.48 & 81.84 & 86.31 & 85.1 & 85.7 & 81.41 & 82.56 & 81.99 & 84.8 & 85.04 & 84.92\\ 
%             & S\textsc{OTA} &  - & - & \textbf{95.68} & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 87.97 & 87.42 & 87.69 & 88.47 & 88.47 & 88.47 & 86.33 & 86.52 & 86.429 & 88.48 & 89.06 & 88.77\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{NCBI-Disease}}}}}
%             & B\textsc{ioBERT} & 86.92 & 89.53 & 88.2 & 87.5 & 90.67 & \textbf{89.05} & 85.75 & 88.6 & 87.15 & 86.32 & 89.16 & 87.72\\ 
%             & M\textsc{imicBERT} & 84.22 & 86.83 & 85.51 & 86.82 & 88.8 & 87.80 & 85.69 & 85.69 & 85.69 & 84.43 & 85 & 84.72\\ 
%             & S\textsc{OTA} &  - & - & 88.60 & - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 86.19 & 89.94 & 88.03 & 86.66 & 90.88 & 88.72 & 86.75 & 88.91 & 87.81 & 86.59 & 88.68 & 87.62\\ 
%              \hline
             
             
%             % \multirow{3}{*}{
%             %     \rotatebox[origin=c]{0}{
%             %         \shortstack{\textbf{\texttt{2009 Medical}}}}}
%             % & B\textsc{ioBERT} & 18.84 & 45.24 & 26.6 & 2.67 & 61.84 & 31.58 & 32.41 & 59.1 & 41.87 & 37.41 & 54.37 & 44.32\\ 
%             % & M\textsc{imicBERT} & 67.36 & 66.75& 66.75\\ 
%             % & S\textsc{OTA} & 67.36 & 66.75& 66.75& - & -& - & -&- & -& - & -&-\\ 
%             % & C\textsc{NNBERT} & 18.04 & 43.29 & 25.47 & 23.3 & 58.75 & 33.36 & 34.68 & 65.48 & 45.34 & 45.89 & 64.11 & 53.49\\ 
%             %  \hline
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{2010 Relations}}}}}
%             & B\textsc{ioBERT} & 93.41 & 94.12 & 93.76 & 89.16 & 92.47 & 90.79 & 93.21 & 94.09 & 93.65 & 93.29 & 94.41 & 93.84\\ 
%             & M\textsc{imicBERT} & 93.09 & 94.38 & 93.73 & 94.85 & 95.76 & 95.3 & 92.69 & 94.07 & 93.38 & 93.1 & 94.19 & 93.64\\ 
%             & S\textsc{OTA} & - & - &  90.25& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 93.42 & 94.13 & 93.77 & 95.27 & 95.91 & \textbf{95.59} & 92.43 & 93.96 & 93.19 & 93.43 & 94.6 & 94.01\\ 
%              \hline
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{2011 Coreference}}}}}
%             & B\textsc{ioBERT} & 93.14 & 92.2 & 92.67 & 93.88 & 94.15 & 94.02 & 92.93 & 92.12 & 92.52 & 93.89 & 93.36 & 93.62\\ 
%             & M\textsc{imicBERT} &93.028 & 92.54 & 92.78 & 94.18 & 94.3 & 94.24 & 92.69 & 92.14 & 92.42 & 93.77 & 93.25 & 93.5\\ 
%             & S\textsc{OTA} & - & - & -& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 93.1 & 92.04 & 92.57 & 94.42 & 94.37 & \textbf{94.40} & 92.32 & 92.09 & 92.21 & 94.23 & 93.67 & 93.95\\ 
%              \hline
             
             
%             \multirow{3}{*}{
%                 \rotatebox[origin=c]{0}{
%                     \shortstack{\textbf{\texttt{2012 Temporal}}}}}
%             & B\textsc{ioBERT} &73.61 & 81.76 & 77.47 & 74 & 70.9 & 72.42 & 73.47 & 81.97 & 77.49 & 73.53 & 83.21 & 78.07\\ 
%             & M\textsc{imicBERT} & 73.89 & 82.27 & 77.86 & 81.57 & 84.76 & 83.13 & 71.01 & 82.27 & 76.22 & 72.44 & 83.74 & 77.68\\ 
%             & S\textsc{OTA} & - & -& 80.91& - & -& - & -&- & -& - & -&-\\ 
%             & C\textsc{NNBERT} & 76.26 & 82.2 & 79.12 & 81.84 & 84.52 & \textbf{83.14} & 73.11 & 82.3 & 77.44 & 75.63 & 83.96 & 79.58\\ 
%              \hline
%             \end{tabular}
%             }
%             \caption{ \textcolor{red}{TODO UDPATE}
%             Precision(P), Recall(R) and F-Measure(F) for all the mentioned datasets using BioBERT and Mimic-TrainedBERT for Context$_1$ (Entity Name), Context$_2$ (Question), Context$_3$ (Definition)  and Context$_4$ (Examples). Bold represents state-of-the-art.  
%                 }
%             \label{tab:eval}
%         \end{table*}  



% % \begin{figure}
% % \centering
% %   \includegraphics[width=\linewidth,height=3cm]{emnlp2020-templates/images/Bertviz_custom.png}
% %   \caption{Query tokens attending to the correct answer \textit{pain} in BERT-CNN model trained with \textit{Question}.}
% %   \label{fig:viz}
% % \end{figure}

% \section{Review comments}
% \subsection{rev1}
% \textbf{What is this paper about, what contributions does it make, what are the main strengths and weaknesses?}
% This work formulates the NER task as a question answering task by adding external knowledge, such as entity definition, entity examples, enabling the model to attend to these text during the prediction. With the experiments focusing on the biomedical domain, the model achieves the state-of-the-art results in 16 out of 18 datasets.
% \textbf{Strengths}
% 1. This work empirically investigates which types of knowledge are better in the setting of question answering based NER, including entity type, question, definition, and examples.
% 2. Achieving the state-of-the-art results in 16 biomedical NER datasets.
% \textbf{Weaknesses}
% 1. Applying question answering to NER is not novel, which has been investigated in [1], [2]. The context concepts in this paper including "definition", "question" and "entity type" match the concepts of “wikipedia”, “rule-based template filling” and “keyword”.
% 2. I did not find results of the baseline model which follows the traditional sequence tagging method on these datasets. These results are important for supporting this new formulation for NER task.
% [1] A Unified MRC Framework for Named Entity Recognition. Xiaoya Li, Jingrong Feng, Yuxian Meng, Qinghong Han, Fei Wu and Jiwei Li
% [2] Query-Based Named Entity Recognition. Yuxian Meng, Xiaoya Li, Zijun Sun and Jiwei Li
% \textbf{Reasons to accept}
% The proposed method achieves the state-of-the-art results in 16 biomedical NER datasets.
% \textbf{Reasons to reject}
% 1. The authors did not justify the novelty of the formulation. See \textbf{weaknesses 1.}
% 2. Some baseline results are missing which are required to support the new question formulation for NER task. See
% weaknesses 2.
% \textbf{Questions for the Authors(s)}
% 1. Instead of using the BIO tagging, what’s the result if the authors use the reading comprehension style decoding method where start and end positions are predicted, as in [1].
% 2. What’s the performance of this model on more general NER datasets, such as ontonotes.
% 3. See weaknesses 1 and 2.
% [1] A Unified MRC Framework for Named Entity Recognition. Xiaoya Li, Jingrong Feng, Yuxian Meng, Qinghong Han, Fei Wu and Jiwei Li
% \subsection{rev2}
% What is this paper about, what contributions does it make, what are the main strengths and weaknesses?
% This paper tries to pose NER as a question answering problem. That is, the input sentence is encoded with 4 different kinds of knowledge: Entity type, template-based question, definition of the entity type, or entity examples. Since the entity type is encoded as part of the input, the possible output labels become only B, I, or O (without typing).
% \textbf{Strengths}: The idea is pretty interesting. Comparing with other methods, the proposed approach performs much better across 7 datasets.
% \textbf{Weaknesses}: The experiments do not really show that external knowledge is useful. When using Definition and Example as context, the performance is much worse. Using Entity or Question as context is essentially the same as adding entity types as part of inputs.
% It would be nice to add a baseline of the standard BERT-based NER model.
% \textbf{Reasons to accept}
% The idea is potentially useful.
% \textbf{Reasons to reject}
% The experiments do not really support the claims.
% \textbf{Questions for the Authors(s)}
% Why is there large difference between "Entity" method and "Question" method? From the example in Table 1, these two methods use essentially the same information since the questions are generated by templates.


% \subsection{rev3}
% \textbf{What is this paper about, what contributions does it make, what are the main strengths and weaknesses?}
% In this paper, the authors attempt to formulate NER task as a multi-answer question answering, and put the training procedure in a multitask learning scenario. The authors take biomedical text as testbed of their proposed framework. This framework utilizes external knowledge to help boost the performance of NER. The authors combined multiple datasets and create the context which is required. Experiments show that the proposed framework outperformed the SOTA approaches.
% \textbf{Strengths}: The core idea of the paper is quite interesting, it shows a possible direction of utilizing external information.
% \textbf{Weakness}: I find it a little hard to follow. If I understand correctly, the framework only detects the boundaries (text span) of entities first, then using QA system to determine the entity type, since the selected entities will be the answers to those "What" questions. Then I don't think this is a "reformulation" of NER, it still follows a routine of "detect first then classify".
% The description of the proposed approach is a little circular, I think the authors should rectify the use of variables, or it just sounds very informal and confusing such as "given the entities, we find the entities", this can be avoided by introducing careful
% usage and reference of variables.
% The authors did not mention multiple label issue, e.g., when answering multiple questions with regard to multiple entities, how do you decide the ultimate label of an entity if it appears in the answer of multiple entity type questions.
% \textbf{Reasons to accept}
% This paper provides a cute idea that we may jointly utilize external knowledge and information from other models.
% \textbf{Reasons to reject}
% The writing is very confusing, particularly some description seems circular. The experiments are conducted on a union of multiple datasets instead of running on each dataset respectively, the performance might not be convincing.
% \textbf{Questions for the Authors(s)}
% How do you determine a label when an entity candidate appears in the answers of multiple questions regarding the entity types?

% \subsection{META REVIEW}

% \textbf{Comments}: This paper formulates NER as a multi-answer question-answering task and supplements a BERT model with background knowledge. While the idea of NER as QA has been recently proposed by other works, this paper specifically applies it to the biomedical domain and shows that multi-tasking is effective in this setting -- showing better performance on 16 datasets out of 18 (the absolute gains are small -- it would have been more convincing if the paper also reported mean and std. dev. across N random seeds).  

% I think the paper contains enough interesting results for a short paper. But, the paper does need some presentation improvement and reorganization (especially moving some important experiment details from supplement to the main draft). As examples: (i) it is unclear if the baselines are also trained by multi-tasking across all datasets. (ii) it is also unclear if the method uses all proposed types of additional contexts jointly. Experiments show results of using each of them individually.
